Charm (and Beauty) Production at the Tevatron

We present recent results on heavy flavour production at Tevatron Run II for typically ~1/fb of analysed proton-antiproton data at a c.m. energy of 1.96 TeV. This includes results on single and correlated open charm and bottom cross sections, charm pair production kinematics, J/psi, psi(2S) and chi cross sections and polarisation measurements in J/psi, psi(2S), Upsilon(1S), and Upsilon(2S).

==> btodst_commands.tex <==
%
%-------------------------------------------------------------------
\newcommand{\prt}[1]{\ensuremath{{\rm #1}}}
\newcommand{\qrk}[1]{\ensuremath{#1}}
%-------------------------------------------------------------------
\newcommand{\Bo}{\prt{B^0}}
\newcommand{\Bob}{\prt{\overline{B^0}}}
\newcommand{\Bh}{\prt{B_{H}}}
\newcommand{\Bl}{\prt{B_{L}}}
\newcommand{\Bso}{\prt{B_{s}^0}}
\newcommand{\Bsob}{\prt{\overline{B_{s}^0}}}
\newcommand{\Bdo}{\prt{B_{d}^0}}
\newcommand{\Bdob}{\prt{\overline{B_{d}^0}}}
\newcommand{\Dst}{\prt{{D}^{\ast}}}
\newcommand{\Dstp}{\prt{{D}^{\ast +}}}
\newcommand{\Dstm}{\prt{{D}^{\ast -}}}
\newcommand{\aI}{\prt{a_1}}
\newcommand{\aIp}{\prt{a_1^+}}
\newcommand{\aIm}{\prt{a_1^-}}
\newcommand{\pion}{\prt{\pi}}
\newcommand{\pip}{\prt{\pi^+}}
\newcommand{\pim}{\prt{\pi^-}}
\newcommand{\Do}{\prt{D^{0}}}
\newcommand{\Dob}{\prt{\overline{D^0}}}
\newcommand{\Ds}{\prt{D_s}}
\newcommand{\Dso}{\prt{D_s^{0}}}
\newcommand{\Dsob}{\prt{\overline{D_s^0}}}
\newcommand{\Kp}{\prt{K^+}}
\newcommand{\Km}{\prt{K^-}}
\newcommand{\Ks}{\prt{K_S}}
\newcommand{\Kl}{\prt{K_L}}
\newcommand{\Jpsi}{\prt{J\!/\!\psi}}

\newcommand{\bbar}{\qrk{b\overline{b}}}

\newcommand{\Dstpi}{\prt{\Dst \pi}}
\newcommand{\Dstpluspi}{\prt{\Dstp \pim}}
\newcommand{\Dstminuspi}{\prt{\Dstm \pip}}

\newcommand{\pis}{\prt{\pi_{\mathrm{slow}}}}
\newcommand{\pif}{\prt{\pi_{\mathrm{fast}}}}
\newcommand{\boldpis}{\ensuremath{\bf \pi_{\mathrm{slow}}}}
\newcommand{\boldpif}{\ensuremath{\bf \pi_{\mathrm{fast}}}}

%-----------------------------------------------------------

\newcommand{\BDmn}{\prt{\Bdo\to \Dstm \pip}}
\newcommand{\BDpl}{\prt{\Bdo\to \Dstp \pim}}
\newcommand{\BbDmn}{\prt{\Bdob\to \Dstm \pip}}
\newcommand{\BbDpl}{\prt{\Bdob\to \Dstp  \pim}}

\newcommand{\cBDmn}{\prt{\Bdo\to \Dstm \pip}}
\newcommand{\cBDpl}{\prt{\Bdo\to {\color{red}\Dstp  \pim}}}
\newcommand{\cBbDmn}{\prt{{\color{red}\Bdob}\to \Dstm \pip}}
\newcommand{\cBbDpl}{\prt{{\color{red}\Bdob}\to {\color{red}{\Dstp \pim}}}}

\newcommand{\DmnDzb}{\prt{\Dstm \to \Dob \pim}}
\newcommand{\DplDz}{\prt{\Dstp \to \Do \pip}}

\newcommand{\DzbK}{\prt{\Dob \to \Kp \pim}}
\newcommand{\DzK}{\prt{\Dob \to \Km \pip}}

\newcommand{\BDmna}{\prt{\Bdo \to \Dstm \aIp}}
\newcommand{\BDpla}{\prt{\Bdo \to \Dstp \aIm}}
\newcommand{\BbDmna}{\prt{\Bdob\to \Dstm \aIp}}
\newcommand{\BbDpla}{\prt{\Bdob\to \Dstp \aIm}}
\newcommand{\BDst}{\prt{\Bdo \to \Dst}}
\newcommand{\BDpi}{\prt{\Bdo \to \Dst\pi}}
\newcommand{\BDa}{\prt{\Bdo \to \Dst \aI}}
\newcommand{\BDpia}{\prt{\Bdo \to \Dst\pi(\aI)}}
\newcommand{\Bpipi}{\prt{\Bdo \to \pip \pim}}
\newcommand{\BsKK}{\prt{\Bso \to K^+ K^-}}
\newcommand{\Bbpipi}{\prt{\Bdob\to \pip \pim}}
\newcommand{\BJpsiK}{\prt{\Bdo \to \Jpsi \Ks}}
\newcommand{\BbJpsiK}{\prt{\Bdob\to \Jpsi \Ks}}
\newcommand{\BsDsK}{\prt{\Bso \to \Ds \prt{K}}}
\newcommand{\BsDspi}{\prt{\Bso \to \Ds \pi}}
%----------------------------------------------------------------
\newcommand{\gam}{\ensuremath{\gamma}}
\newcommand{\bet}{\ensuremath{\beta}}
\newcommand{\phimix}{\ensuremath{\phi_{\mathrm{mix}}}}
\newcommand{\dckm}{\ensuremath{\phimix - \gam}}
\newcommand{\Dstrong}{\ensuremath{\Delta_{\mathrm{qcd}}}}
\newcommand{\etta}{\ensuremath{\eta}}
\newcommand{\ettabar}{\ensuremath{\overline{\eta}}}
\newcommand{\Imetta}{\ensuremath{\mathsf{Im}\!\left(\etta\right)}}
\newcommand{\Imettabar}{\ensuremath{\mathsf{Im}\!\left(\ettabar\right)}}
\newcommand{\sinplus}{\ensuremath{\sin\!\left(\Dstrong + \left(\dckm\right)\right)}}
\newcommand{\sinminus}{\ensuremath{\sin\!\left(\Dstrong - \left(\dckm\right)\right)}}
\newcommand{\sinpm}{\ensuremath{\sin\!\left(\Dstrong \pm \left(\dckm\right)\right)}}
\newcommand{\modetta}{\ensuremath{\left|\etta\right|}}
\newcommand{\modettabar}{\ensuremath{\left|\ettabar\right|}}
\newcommand{\modettasq}{\ensuremath{\left|\etta\right|^2}}
%
\newcommand{\siggam}{\ensuremath{\sigma_{\gamma}}}
\newcommand{\dm}{\ensuremath{\Delta\!m}}

\newcommand{\mtag}{\ensuremath{\omega_{\mathrm{tag}}}}

\newcommand{\sIIb}{\ensuremath{\sin\!\left(2\beta\right)}}

%---------------------------------------------------------------
\newcommand{\epstag}{\ensuremath{\epsilon_{\mathrm{tag}}}}
\newcommand{\ptag}{\ensuremath{P_\mathrm{tag}}}
%
%---------------------------------------------------------------
\newcommand{\ppslow}{\ensuremath{\vec{p}_{\pis}}}
\newcommand{\ppfast}{\ensuremath{\vec{p}_{\pif}}}
\newcommand{\pDst}{\ensuremath{\vec{p}_{\Dst}}}
\newcommand{\pDo}{\ensuremath{\vec{p}_{\Do}}}
\newcommand{\pBo}{\ensuremath{\vec{p}_{\Bo}}}
%
%---------------------------------------------------------------
\newcommand{\dal}{\ensuremath{\Delta\!\alpha}}
\newcommand{\alo}{\ensuremath{\alpha_{\circ}}}
\newcommand{\dpvec}{\ensuremath{\left|\Delta\!\vec{p} \right|}}
%
%---------------------------------------------------------------
\newcommand{\Vckm}{\ensuremath{V_{\mathrm{CKM}}}}
%
%---------------------------------------------------------------






